WILDCHAT-50M: A Deep Dive Into the Role of Synthetic Data in Post-Training

Language model (LLM) post-training, from DPO to distillation, can refine behaviors and unlock new skills, but the open science supporting these post-training techniques is still in its infancy. One limiting factor has been the difficulty of conducting large-scale comparative analyses of synthetic data generating models and LLM judges. To close this gap, we introduce WILDCHAT-50M, the largest public chat dataset to date. We extend the existing WildChat dataset to include responses not only from GPT, but from over 50 different open-weight models, ranging in size from 0.5B to 104B parameters. We conduct an extensive comparative analysis and demonstrate the potential of this dataset by creating RE-WILD, our own public SFT mix, which outperforms the recent Tulu-3 SFT mixture from Allen AI with only 40% as many samples. Our dataset, samples and code are available at https://github.com/penfever/wildchat-50m.

==> figures/at_a_glance.tex <==
\begin{tikzpicture}[
    box/.style={
        rectangle,
        rounded corners=15pt,
        minimum width=6cm,
        minimum height=3cm,
        draw=white,
        fill=white,
        drop shadow={shadow xshift=0.3ex, shadow yshift=-0.3ex},
        text width=5.5cm,
        align=left
    },
    number/.style={
        circle,
        minimum size=1cm,
        font=\large\bfseries,
        text=white
    }
]

% Center circle background
\node[circle, draw=gray!20, fill=white, minimum size=4cm, drop shadow] at (0,0) {};
% Text on top
\node[text width=3cm, align=center] at (0,2.75) {\textbf{WildChat-50m}\\[0.2cm]\textbf{\textcolor{red}{At a Glance}}};

% Circular segments
\foreach \angle/\col in {45/myteal, 135/mytan, 225/mytan, 315/myteal} {
    \path[fill=\col] (0,0) -- (\angle:2cm) arc (\angle:\angle+80:2cm) -- cycle;
}

% Boxes with content
\node[box] at (-5,5) {
    \textbf{01}
    \vspace{0.2cm}
    
    \textbf{54 models (19 unique pretrained, 35 unique post-trained)}
    
    \tikz\node[font=\Large] at (0,-1.5) {\faUser};
};

\node[box] at (5,5) {
    \textbf{02}
    \vspace{0.2cm}
    
    \textbf{1 Mn conversations per model}
    
    \tikz\node[font=\Large] at (0,-1.5) {\faComments};
};

\node[box] at (-5,-5) {
    \textbf{03}
    \vspace{0.2cm}
    
    \textbf{5 models judged, 12 judgment factors}
    
    \tikz\node[font=\Large] at (0,-1.5) {\faAdjust};
};

\node[box] at (5,-5) {
    \textbf{04}
    \vspace{0.2cm}
    
    \textbf{Up to 20,000 tokens per response}
    
    \tikz\node[font=\Large] at (0,-1.5) {\faBicycle};
};
\label{fig:wc50m-overview}
\end{tikzpicture}
\clearpage
